TreeQN and ATreeC: Differentiable Tree-Structured Models for Deep Reinforcement Learning

Combining deep model-free reinforcement learning with on-line planning is a promising approach to building on the successes of deep RL. On-line planning with look-ahead trees has proven successful in environments where transition models are known a priori. However, in complex environments where transition models need to be learned from data, the deficiencies of learned models have limited their utility for planning. To address these challenges, we propose TreeQN, a differentiable, recursive, tree-structured model that serves as a drop-in replacement for any value function network in deep RL with discrete actions. TreeQN dynamically constructs a tree by recursively applying a transition model in a learned abstract state space and then aggregating predicted rewards and state-values using a tree backup to estimate Q-values. We also propose ATreeC, an actor-critic variant that augments TreeQN with a softmax layer to form a stochastic policy network. Both approaches are trained end-to-end, such that the learned model is optimised for its actual use in the tree. We show that TreeQN and ATreeC outperform n-step DQN and A2C on a box-pushing task, as well as n-step DQN and value prediction networks (Oh et al. 2017) on multiple Atari games. Furthermore, we present ablation studies that demonstrate the effect of different auxiliary losses on learning transition models.

==> core/2_background.tex <==
\section{Background}
\label{sec:background}
We consider an agent that learns to act in a Markov Decision Process (MDP), with
the goal of maximising its expected discounted sum of rewards $R_t =
\sum_{t=0}^{\infty}\gamma^t r_t$.
It does so by learning a policy $\pi(\state)$ that maps
states $\state \in \set{S}$ to actions $a \in \set{A}$.
The state-action value function ($Q$-function) is defined as $Q^{\pi}(\state,a)
= \E_\pi \left[R_t | \state_t = \state,a_t = a \right]$; the optimal
$Q$-function
is $Q^{*}(\state,a) = \max_{\pi} Q^{\pi}(\state,a)$.

In the Bellman optimality equation $Q^*$ is recursively defined as
\[Q^*(\state,a) =
\mathcal{T}Q^*(\state,a) \equiv r(\state,a) + \gamma \sum_{\state'}
P(\state'|\state,a) \max_{a'} Q^*(\state', a'),
\]
where $P$ is the MDP state  transition function and $r$ is a reward function,
which for simplicity we assume to be deterministic.
$Q$-learning \citep{watkins1992q} uses a single-sample approximation of the
contraction operator $\mathcal{T}$ to iteratively improve an estimate of $Q^*$.

In deep $Q$-learning \citep{mnih2015human}, $Q$ is represented by a deep neural
network with parameters $\theta$, and is improved by regressing $Q(\state,a)$
to a target $r + \gamma \max_{a'} Q(\state',a';\theta^{-})$, where
$\theta^{-}$ are the parameters of a target network periodically copied from
$\theta$.

We use a version of $n$-step $Q$-learning
\citep{mnih2016asynchronous} with synchronous environment threads.
In particular, starting at a timestep $t$, we roll forward $n_\text{env} = 16$
threads for $n = 5$ timesteps each.
We then bootstrap off the final states only and gather all $n_\text{env} \times
n = 80$
transitions in a single batch for the backward pass, minimising the loss:
\begin{equation}
  \label{eq:qloss}
\mathcal{L}_\text{nstep-Q} = \sum_\text{envs}\sum_{j=1}^{n}\left(\sum_{k=1}^{j}
\left[
\gamma^{j-k}r_{t+n-k}\right] +
\gamma^j\max_{a'} Q\left(\state_{t+n},a',\theta^{-}\right) -
Q\left(\state_{t+n-j},a_{t+n-j},\theta\right) \right)^2.
\end{equation}
If the episode terminates, we use the remaining episode return as the target,
without bootstrapping.

This algorithm's actor-critic counterpart is A2C, a
synchronous variant of A3C \citep{mnih2016asynchronous} in which a policy $\pi$
and state-value function $V(s)$ are trained using the gradient:
\begin{multline}
\label{eq:ac_loss}
\Delta\theta = \sum_\text{envs}\sum_{j=1}^{n} \nabla_{\theta_\pi} \log
\pi(a_{t+n-j}|s_{t+n-j}) A_j(s_{t+n-j}, a_{t+n-j}) + \beta H(\pi(s_{t+n-j})) \\
+ \alpha \nabla_{\theta_V} A_j(s_{t+n-j}, a_{t+n-j})^2 ,
\end{multline}
where $A_j$ is an advantage estimate given by $\sum_{k=1}^{j}
\gamma^{j-k}r_{t+n-k} + \gamma^j V(\state_{t+n}) - V(\state_{t+n-j})$, $H$ is
the policy entropy, $\beta$ is a hyperparameter tuning the degree of
entropy regularisation, and $\alpha$ is a hyperparameter controlling the
relative learning rates of actor and critic.

These algorithms were chosen for their simplicity and reasonable wallclock
speeds, but TreeQN can also be used in other algorithms, as described in
Section \ref{sec:training}.
Our implementations are based on OpenAI Baselines \citep{baselines}.

\begin{wrapfigure}{R}{5cm}
  \centering
    \begin{tikzpicture}
      \pgfmathsetseed{2}
      \name{st}{\rep{3}}
      \node[below = 0cm of st] {$\istate_t$};

      \node[] (S) at (-2, 0) {$\state_t$};
      \draw[-latex, very thick] (S) -- (st);
      \node[rotate=90, anchor=center, draw, very thick, rectangle, text
      width=1.5cm, text centered, rounded corners, nice-purple,
      fill=nice-purple!10] at (-1, 0) {\small$\module{encode}$};

      \node[] (Q) at (2, 0) {$Q$};
      \draw[-latex, very thick] (st) -- (Q);

      \node[rotate=90, anchor=center, draw, very thick, rectangle, text
      width=1.5cm, text centered, rounded corners, nice-blue,
      fill=nice-blue!10] at (1, 0) {\small$\module{evaluate}$};
    \end{tikzpicture}
  \caption{High-level structure of DQN.}
  \label{fig:dqn}
  \vspace{-2mm}
\end{wrapfigure}


The canonical neural network architecture in deep RL
with visual observations has a series of convolutional layers followed by two
fully connected layers, where the final layer produces one output for each
action-value. We can think of this network as first calculating an encoding $\istate_t$
of the state $\state_t$ which is then evaluated by the final layer to estimate
$Q^*(\state_t,a)$ (see \cref{fig:dqn}).

In tree-search on-line planning, a look-ahead tree of possible future states is
constructed by recursively applying an environment model.
These states are typically evaluated by a heuristic, a learned value function,
or Monte-Carlo rollouts.
Backups through the tree aggregate these values along with the immediate
rewards accumulated along each path to estimate the value of taking
an action in the current state.
Our paper focuses on a simple tree-search with a deterministic transition
function and no value uncertainty estimates, but our approach can be extended
to tree-search variants like UCT \citep{kocsis2006bandit,silver2016mastering} if the components remain
differentiable.


==> figures/X.tex <==
\relax 
\@setckpt{../include/tikzmacros.tex}{
\setcounter{page}{2}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{sapage}{0}
\setcounter{part}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{ContinuedFloat}{0}
\setcounter{subfigure}{0}
\setcounter{subtable}{0}
}


==> figures/q.tex <==
\relax 
\@setckpt{../include/tikzmacros}{
\setcounter{page}{2}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{0}
\setcounter{mpfootnote}{0}
\setcounter{sapage}{0}
\setcounter{part}{0}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{ContinuedFloat}{0}
\setcounter{subfigure}{0}
\setcounter{subtable}{0}
}


==> figures/tikzmacros.tex <==
% scaling
\newcommand{\scale}[2]{
  % \begin{scope}[transform canvas={scale=#1}]
  \begin{scope}[scale=#1]
    #2
  \end{scope}
}

% naming
\newcommand{\name}[2]{
  \begin{scope}[local bounding box=#1]
    #2
  \end{scope}
}

% relative positioning
\newcommand{\at}[3]{
  \begin{scope}[shift={(#1,#2)}]
    #3
  \end{scope} 
}


\newcommand{\grid}[4]{
    \draw[fill=white, opacity=0.5] (#1, #2) rectangle (#3, #4);
    \draw[help lines, red, opacity=0.5] (#1, #2) grid (#3, #4);
    \foreach \x in {#1,...,#3} {
      \foreach \y in {#2,...,#4} {
        \node[anchor=east] at (\x+0.1,\y+0.1) {\tiny\color{red}\x};
        \node[anchor=west] at (\x-0.1,\y+0.1) {\tiny\color{red}\y};
      }
    }
}

% neural 
\newcommand{\rep}[1]{
    \begin{scope}[scale=0.5]
        \begin{scope}[shift={(0,-#1/2.0)}]
            \draw[very thick, fill=white] (-0.5, 0) rectangle (0.5, #1);
            \foreach \x in {1,...,#1} {
                \draw[very thick] (0, \x-0.5) circle (0.44);
            }
        \end{scope}
    \end{scope}
}
